Tidally locked rotation of the dwarf planet (136199) Eris discovered from long-term ground based and space photometry

The rotational states of the members in the dwarf planet - satellite systems in the transneptunian region are determined by the formation conditions and the tidal interaction between the components, and these rotational characteristics are the prime tracers of their evolution. Previously a number of authors claimed highly diverse values for the rotation period for the dwarf planet Eris, ranging from a few hours to a rotation (nearly) synchronous with the orbital period (15.8 d) of its satellite, Dysnomia. In this letter we present new light curve data of Eris, taken with $\sim$1-2m-class ground based telescopes, and with the TESS and Gaia space telescopes. TESS data could not provide a well-defined light curve period, but could constrain light curve variations to a maximum possible light curve amplitude of $\Delta m$ $\leq$ 0.03 mag (1-$\sigma$) for P $\leq$ 24 h periods. Both the combined ground-based data and the Gaia measurements unambiguously point to a light curve period equal to the orbital period of Dysnomia, P = 15.8 d, with a light curve amplitude of $\Delta m$ $\approx$ 0.03 mag, i.e. the rotation of Eris is tidally locked. Assuming that Dysnomia has a collisional origin, calculations with a simple tidal evolution model show that Dysnomia has to be relatively massive (mass ratio of q = 0.01--0.03) and large (radius of $R_s$ $\geq$ 300 km) to slow down Eris to synchronized rotation. These simulations also indicate that -- assuming tidal parameters usually considered for transneptunian objects -- the density of Dysnomia should be 1.8-2.4 $g cm^{-3}$, an exceptionally high value among similarly sized transneptunian objects, putting important constraints on the formation conditions.

==> eris_rot_ans_rev_R1.tex <==
Dear Dr Szakáts,

Your paper "Tidally locked rotation of the dwarf planet (136199) Eris discovered from long-term ground based and space photometry" was submitted to a referee who recommends publication after revision (see enclosed report and marked-up copy).

Please see also additional comments from myself below.

Please take the referee's comments and suggestions into account when revising your work and send us the new version. Instructions for resubmission can be found at https://mmsaanda.obspm.fr/is/aa/resubmit_a_paper.php. Your author ID number is 31277.

- In your cover letter, please indicate precisely all of the changes made in the revised version; there should be two PDF files (one in printer format and the other in referee format).

- Mark all of the changes clearly (using boldface or latexdiff) in your manuscript.

The deadline for the submission of your revised version is one month from today.

With best regards,

Emmanuel Lellouch A&A Editor

------------------

Referee Report ( + attached annotated copy)

omments for the author

Overall this is a well thought out and clearly written paper presenting data investigating the rotation period of the dwarf planet Eris using four different datasets. I appreciate that you did the analysis on each dataset individually looking somewhat for consistency across results. I really like the contour plot (eg. Fig 1) of amplitude vs. period, that was a nice way to look at the various possible results both visually and statistically.  I also appreciate that you did the tidal evolution model for comparison although I think of that as somewhat contrived since the model is forward looking and from the data perspective we are backwards looking. It is a decent consistency check, I'll admit.
I don't have any major comments on the science. I would definitely refer to it in the future so a letter is ok but I don't really see any reason to expedite it. It is an important contribution, but not a landmark result. I find the format of all the analysis in appendices instead of in the text rather cumbersome for fully digesting the paper. I'm guessing that it is the letter format and it is what it is, more a matter of style than preference. It is well written and cross-referenced, but I would really recommend that all the appendix information be in the main text -- if that is the format for a Main Journal article then, while it is OK as a letter, I would highly recommend revising it as a Main Journal article.
I am attaching an annotated PDF with a handful of highlights, edits and a few comments for added references or discussion.

------------------------

Editor's notes

General comments
I agree with the referee that the format with all the details relegated to the appendices is a little cumbersome (in additions, some parameters appear to be defined precisely in the appendix but not in the main text, see below), but I will not object continuing considering the paper as a Letter and keeping the present format if you prefer so. In that case, however, please note that A & A appendices do not go to language editor and are published camera-ready, so you should take special care in their layout (typos, figure quality etc., Fig. 4 and A.1 in particular need replacement).
Tables must have a short title, above the table, with a footnote below the table for the rest of the caption. (Tables A.1, A.2, A.5.)
**A: Fig. 4 and A.1 have been replaced with higher resolution figures.
**A: The tables have been reformatted with a caption at the top and with footnotes.

Specific comments
- Abstract: the conclusion on the density seems too definitive to me, given that (Sect 3) you find solutions at rho ~ 1 for low values of Q (10). Although such a low Q may be unlikely, more caution should be exercised. Same in the Conclusion section. In relation to this: as you may know, measuring masses and therefore densities of TNO from the wobble in astrometric radio data is being attempted (2019AAS...23335412B). Although results aren't available yet, you might want to add somewhere a comment that combining such measurements with the tidal analysis presented here could perhaps constrain Q.
** A: we put an additional sentence at the end of Sect. 3. and an additional note in the abstract that the 1.8-2.4 g/cm3 density value is obtained using the canonical tidal parameters.  

- The paper's sub-title could be more specific. 
**A: The paper has no 'subtitle' so we guess that the reviewer refers to the second half of the title "discovered from...". Indeed, the instruments, mainly Gaia, and at some level TESS, could be mentioned here, but their weight and role could be seen only after reading the paper and we did not want a misleading title. So we would like to keep the title as it is now. 

- Sect 2.2 and Fig. 1. C(P, Delta_m) should be defined here also. What is the necessity to subtract min (C) in Fig. 1? (it is not done in Fig. A.4)? Please add color bar and remove figure grids (per A & A figure policy). Same for Fig. A.4.
** A: We added color bars and removed the grids in the case of both figures. Note that now both figures represent C(P,dm) (without the -min(C(P,dm))), and therefore the appearance of the figures are slightly different. Also note that the C(P,dm) levels are different in the case of Fig. 1 and Fig. A4 due to different data and uncertainties, and that C(P,dm) is not normalized. 

- Sect 2.2, 2.3. What is the significance level of the inferred 15.8 d period? Fig. A2 (P=58 hours, for which you quote a 1.8 sigma confidence) looks even more convincing than Fig. 2 (15.8 day). It was also not completely clear to me if the method described in A.5 was applied to the whole set of ground based data simultaneously but separately for Gaia, or if everything was combined.
**A: The Gaia data was evaluated separately from the ground-based data as it contained enough data points and covered a sufficiently long period that it could be used for period determination in the few days - synchronized rotation range. The significance of the 15.8d period, based on the Gaia data only and using the residual spectrum is estimated to be 5.5 sigma. 

- page 3, "Therefore we argue". Italics for underlining are not permitted by the publisher.
**A: The text is not in italics anymore.

- the argument at the end of Sect. 2 is weakened by the fact that methane ice also has absorption bands (weaker than IR, admittedly) in the optical. Given that, I wonder if it is reasonable to associate a small photometric variation (0.03 mag) and the huge color variation (0.58 mag) ?
**A: A quantitative assessment of a possible significant colour variation is beyond the scope of this paper. However, the Eris reflectance spectrum presented by Alvarez-Candal et al. (2011,2020) indeed shows a huge reflectance change from either the visible (~R) or the J-band to the H-band. If this strong methane feature is not present in some rotational phases, the visible-H or J-H colours could be rather different from those of other phases. The large variation in the H-band cannot likely be associated with purely instrumental/calibration issue, however, cross-calibration issues between the different instruments may reduce this difference. (see also the comment in the annotated PDF)

- Sect 3. P_pf does not appear to be defined.
**A: We added $P_{pf}$ at an additional place in Sect. 3, par. 2 for clarity 

- Sect 3, end of 4th paragraph. It would be good to cite the albedo of Dysnomia found by Brown and Butler 2018.
**A: the sentence has been codified to include the BB18 albedo as well

- p. 3, last line; and Fig. 4. What does +/-10\% mean? Aren't the Q values in the model exactly defined?
**A: The data points presented in Fig. 4 are selected for three speific Qp values, 50, 100 and 200. However, in our simulations Qp values are assigned randomly, so for these three cases we selected Qp=50(+/-)5, Qp=100(+/-)10 and Qp=200(+/-)20, i.e. in a range of +/- 10% for all three cases.  

- Fig. 3. "blue symbols...". This does not appear obviously consistent with the inset which says "Ppf all". "corotation" --> "synchronization" (for consistency with the rest of the paper).
**A: Replaced fig 3. with a new version, where corotation was changed to synchronization. also, fig A.7. was changed the same way.

- Sect 4. "The non-Keplerian orbit of Dysnomia could also be caused by a non-spherical shape of the satellite". Is a mass ratio even of 1/30 - 1/50 sufficient for the shape of the satellite to be important?
**A: This was one of the explanations in the Holler et al. (2021) paper for the non-Keplerian orbit of Dysnomia which is not discussed any further in this paper, so we do now know what physical process has Holler et al. associated with the irregular shape. We just listed it along with the other possible reasons. In one hand, however, we think -- as it is discussed in the paper -- that at a size of D>600km Dysnomia is expected to be fairly round, based on the expected shapes of similarly size objects in the main belt and in the Kuiper belt. On the other hand, even in the case of synchronized rotation (i.e. 1:1 spin-orbit resonance for both members of the system) small librations around the equlibrium configuration might occur, especially in the case of a non-spherical satellite which can also lead to a precession of the satellite orbit, i.e. a "non-Keplerian" orbit of Dysnomia (e.g. Murray & Dermott, 2000). While this is a very interesting phenomenon to follow, it is definitely beyond the scope of this present paper. 

- Eq A.2 and a few lines below. k_2 or k_2p ?:
**A: The sentence "The second order tidal Love number k2... " is a general one, not specific for Eris, therefore the 'p' subscript is not used here.  

- Fig A.5. Please use larger fonts for axis values and titles.: 
**A: the figure has been replaced with a new version with larger fonts and labels

- The appendix ends abruptly. Especially, Fig. A7 is not refered to nor explained.
**Ą: We included a new paragraph on Fig. A7. 

- typos: nigth, Dysnmoia                                            
**A: corrected

%%%%%%%%%%%%%%%%%%%%%

Comments from the annotated PDF (typos and grammatical issues have been corrected, as marked by the reviewer, but are not listed here): 

- Page 1: Also consider referencing: Brown et al. 2006 AJ, 639,L43: 
**A: included

- Page 2: How much time did the full dataset span and what is the geometric change for Eris during this time? I assume small since it’s far from the Sun, but worth noting in numeric form. 
**A: We included additional data in the caption of Table A3, and additional sentences on the aspect angle changes at the end of Sect. A3. 

- Page 3: additional references are included in the text on giant collisions (Sect. 3, par. 1)

- Page 7: 2 min or 20 min: text has been replaced here with a hopefully more clear one.




